Rectification from Radially-Distorted Scales

This paper introduces the first minimal solvers that jointly estimate lens distortion and affine rectification from repetitions of rigidly transformed coplanar local features. The proposed solvers incorporate lens distortion into the camera model and extend accurate rectification to wide-angle images that contain nearly any type of coplanar repeated content. We demonstrate a principled approach to generating stable minimal solvers by the Grobner basis method, which is accomplished by sampling feasible monomial bases to maximize numerical stability. Synthetic and real-image experiments confirm that the solvers give accurate rectifications from noisy measurements when used in a RANSAC-based estimator. The proposed solvers demonstrate superior robustness to noise compared to the state-of-the-art. The solvers work on scenes without straight lines and, in general, relax the strong assumptions on scene content made by the state-of-the-art. Accurate rectifications on imagery that was taken with narrow focal length to near fish-eye lenses demonstrate the wide applicability of the proposed method. The method is fully automated, and the code is publicly available at https://github.com/prittjam/repeats.

==> rebuttal/experiments.tex <==
test


==> rebuttal/responses.tex <==
\textbf{AR1: \emph{The language of the paper is quite poor.}}
The comment conflicts with AR3, but the authors agree that the ideas
can be more cleanly distilled for improved clarity. We will improve
the concision of the paper for the camera-ready version.

\textbf{AR1: \emph{one can always use a separate self-calibration step . . .  to determine. . . camera intrinsics.}} 
Self calibration is limited to scene planes that contain known
specialized structure (\eg orthogonal lines or identical circles), so
it is not a reliable approach. In applications where there are unknown
camera types and scene content, which is common for imagery downloaded
from the Internet, self-calibration is not applicable or difficult,
since specialized structure must be detected and verified in the
presence of lens distortion. This unconstrained context is the
motivation for the significant and recent research output for joint
estimation of camera extrinisics and intrinsics in the
state-of-the-art.

\textbf{AR1: \emph{A basis sampling technique proposed in [13] needs
    to be used to deal [with stability issues]. ...the current
    approach appears to require also good luck in finding a suitable
    basis.}}
It is well known that some problems (systems of equations) may lead to
unstable GB solvers; however, the instability does not arise from the
the problem formulation, rather the instability is introduced by the
GB method used for solving the system equations. \Eg, for a selected
basis, the polynomials that are generated from the ideal may be nearly
linearly dependent, which may cause an unstable solver to be
generated. However, for a different basis, there will likely be
different polynomials generated which may result in a more stable
solver. In fact, this observation is leveraged in one of the
contributions of the paper: the objective of the basis-sampling
strategy of \cite{Larsson-CVPR18} was modified to maximize for
stability instead of to minimize for size. Rather than ``good luck'',
this is a principled approach that, given a sufficient sample size,
will generate a stable solver. Furthermore, the proposed solvers are
the first to be generated using stability maximization. Referring to
Fig 2 the basis sampled solvers demonstrate superior stability and
referring to the right panel, significantly better robustness to noise
than to the solvers of Pritts \etal \cite{Pritts-ARXIV17} for
distorted conjugate translations, which is less general than the
proposed problem.

\textbf{AR1: \emph{...the practical importance is quite limited. the
    solver that assumes known distortion is the most important
    practical contribution because it is simple, fast, and the number
    of possible solutions is low.}}
With increasing popularity of wide-angle cameras it's important to
have solvers considering radial distortion. We showed that considering
radial distortion only in final optimization step may lead to
incorrect results. Moreover, it's not usually possible to calibrate
the camera apriori (see above). Regarding the number of possible
solutions.  Usually (97\% of cases in experiments) only a single
solution is feasible in our solutions (this is even less that the
number of feasible solutions of the solver without radial
distortion). Moreover, thanks to the structure of our solvers we can
use efficient Sturm sequences and searching only for eigenvalues
(solutions) in some feasible interval (actually only one solution).

\textbf{AR2: \emph{...the output is useful . . . it feels like the
    problem is being attacked in its most difficult form, using a
    single image."}}
The problem formulation was to work on web imagery, which results in a
difficult and ill-posed estimation, but the the method
gives impressive results because of the ...

and the solvers can be be fused with the
sensor data that AR2 suggests would be useful.

